SymPKF: a symbolic and computational toolbox for the design of parametric Kalman filter dynamics

Recent researches in data assimilation lead to the introduction of the parametric Kalman filter (PKF): an implementation of the Kalman filter, where the covariance matrices are approximated by a parameterized covariance model. In the PKF, the dynamics of the covariance during the forecast step relies on the prediction of the covariance parameters. Hence, the design of the parameter dynamics is crucial while it can be tedious to do this by hand. This contribution introduces a python package, SymPKF, able to compute PKF dynamics for univariate statistics and when the covariance model is parameterized from the variance and the local anisotropy of the correlations. The ability of SymPKF to produce the PKF dynamics is shown on a non-linear diffusive advection (Burgers equation) over a 1D domain and the linear advection over a 2D domain. The computation of the PKF dynamics is performed at a symbolic level, but an automatic code generator is also introduced to perform numerical simulations. A final multivariate example illustrates the potential of SymPKF to go beyond the univariate case.

==> makefile <==
# Liste des .pdf du projet
PDF=paper.pdf pres.pdf poster.pdf

# Variable d'environnement 
REP=$(shell pwd | awk -F / '{print $$NF }')

# Commande de compilation
LATEX = pdflatex -interaction=batchmode
#LATEX = pdflatex 
BIBTEX = bibtex -terse
#JABREF = java -jar /usr/share/jabref/jabref
JABREF = /opt/jabref/bin/JabRef

#BIBTEX = bibtex
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
UNDEFINED = "((Reference|Citation).*undefined)|(Label.*multiply defined)"
	#Dépendance pour les .pdf
TEX=$(PDF: .pdf = .tex)

#
#	Commande de compilation
#
pdffiles: $(PDF)

# Commande de compilation
%.pdf : %.tex
	@echo "Compilation du tex"
	@$(LATEX) $<
	# If file `database.bib` is present then extract bibliography from it
#ifeq ("$(wildcard database.bib)","database.bib")
#	@$(JABREF) -a $*,$*_database database.bib -n > jabref.log
#endif
	#@makeindex $*
	@# Etape de compilation suivant la nécessité.
	@if egrep -q $(RERUN) $*.log ; then echo "passe BibTex/LaTeX" ;\
	$(BIBTEX) $* ; $(LATEX) $<;  fi
	@if egrep -q $(RERUN) $*.log ; then echo "passe BibTex/LaTeX" ;\
	$(BIBTEX) $* ; $(LATEX) $<;  fi
	@if egrep -q $(UNDEFINED) $*.log ; then echo "passe Complémentaire";\
	$(BIBTEX) $* ; $(LATEX) $<;  fi
	@# Vérification de la présence de toute la biblio.
	@egrep -i $(UNDEFINED) $*.log || echo "Dépendance biblio non manquante"
	@exit 0

save:
	make clean
	cd .. ; tar --dereference -cvzf $(REP).tgz $(REP) ; horodate $(REP).tgz
clean:
	rm -f *.dvi *.ps *.log *.aux *.out  *.idx *.toc *.blg *.bbl \
		*.ind *.ilg *.nav *.snm
	rm -f *_database.bib *_database.bib.bak
	rm -f `find | grep .*~`
cleanall: clean
	rm -f *.pdf
header:
	ln -sf ~/work/newdoc/latex/header.tex
	ln -sf ~/work/newdoc/latex/header-private.sty
	ln -sf ~/work/newdoc/latex/header-pres.tex
	ln -sf ~/work/newdoc/latex/set_demo
	ln -sf ~/work/bibliodatabase/database.bib
install:
	cp -f ~/work/newdoc/latex/ametsoc.* .
	cp -f ~/work/newdoc/latex/widetext.sty .
	cp -f ~/work/newdoc/latex/beamer* .
	cp -rf ~/work/newdoc/latex/logo .
	cp -i ~/work/newdoc/latex/paper.tex .
	cp -i ~/work/newdoc/latex/pres.tex .
	cp -i ~/work/newdoc/latex/poster.tex .
	cp -f ~/work/newdoc/latex/.gitignore .
	make header
	mkdir figures
	mkdir src
	mkdir version
update:
	cp -f ~/work/newdoc/latex/makefile .

subdatabase:
	@$(JABREF) -n -a paper,paper_database database.bib  > jabref.log


#
#  Export in asimpler form
#
EXPORT_DIR = ./tmp/export_paper/

export:
	mkdir -p $(EXPORT_DIR)
	cp ./paper.tex ./makefile ./widetext.sty  \
		./paper_database.bib ./ametsoc.bst $(EXPORT_DIR)
	# Don't load figures for export.
	./set_demo ./header-private.sty $(EXPORT_DIR)header-private.sty
	

#
#  Construct difference file and prepare compilation for editting
#

DIFF_DIR = ./tmp/diff/
VERSION_OF_REFERENCE = ./version/paper.tex

paper_diff:
	# 1. Create directory for diff.
	mkdir -p $(DIFF_DIR)
	# 2. Copy local files for the compilation
	cp ./makefile ./widetext.sty  \
		./paper_database.bib ./ametsoc.bst $(DIFF_DIR)
	# 3. Don't load figures for export.
	./set_demo ./header-private.sty $(DIFF_DIR)header-private.sty
	# 3. Create the `diff file` 
	latexdiff $(VERSION_OF_REFERENCE) ./paper.tex > $(DIFF_DIR)paper.tex
	

